Benchmarking Table Comprehension In The Wild

Large Language Models (LLMs), while being increasingly dominant on a myriad of knowledge-intensive activities, have only had limited success understanding lengthy table-text mixtures, such as academic papers and financial reports. Recent advances of long-context LLMs have opened up new possibilities for this field. Nonetheless, we identify two roadblocks: (1) Prior benchmarks of table question answering (TableQA) have focused on isolated tables without context, making it hard to evaluate models in real-world scenarios. (2) Prior benchmarks have focused on some narrow skill sets of table comprehension such as table recognition, data manipulation/calculation, table summarization etc., while a skilled human employs those skills collectively. In this work, we introduce TableQuest, a new benchmark designed to evaluate the holistic table comprehension capabilities of LLMs in the natural table-rich context of financial reports. We employ a rigorous data processing and filtering procedure to ensure that the question-answer pairs are logical, reasonable, and diverse. We experiment with 7 state-of-the-art models, and find that despite reasonable accuracy in locating facts, they often falter when required to execute more sophisticated reasoning or multi-step calculations. We conclude with a qualitative study of the failure modes and discuss the challenges of constructing a challenging benchmark. We make the evaluation data, judging procedure and results of this study publicly available to facilitate research in this field.

==> table/table_intro_sample.tex <==
% \begin{table}[h]
% % \centering
% % \begin{tabular}{|p{0.15\textwidth}|p{0.25\textwidth}|p{0.25\textwidth}|p{0.25\textwidth}|}
% % \hline
% % \textbf{Difficulty} & \textbf{Question} & \textbf{Answer} & \textbf{Reference CoT steps} \\
% % \hline
% % Easy & \textbf{How much} are the total commitments expiring within 1 year as listed in the table? & \$721 million. & - \\
% % \hline
% % Medium & \textbf{Calculate} the difference in the adjusted operating margin between fiscal 2022 and fiscal 2023. & 0.2\% & ... Calculate difference: 
% %    15.4\% - 15.2\% = 0.2\% \\
% % \hline
% % Hard & \textbf{Assess the impact} of capital expenditures on the trend of free cash flow over the period from 2021 to 2023. & Increased capital expenditures from 2021 to 2023 do not strictly correlate with ... & 1. Define relationship between free cash flow and capital expenditures
% % ... \\
% % \hline
% % \end{tabular}
% % \caption{Sample Questions, Answers, and Steps by Difficulty Level}
% % \label{tab:samples}
% % \end{table}
